Ultra-Flat Galaxies Selected from RFGC Catalog. II. Orbital Estimates of Halo Masses

We used the Revised Flat Galaxy Catalog (RFGC) to select 817 ultra-flat (UF) edge-on disk galaxies with blue and red apparent axial ratios of $(a/b)_B > 10.0$ and $(a/b)_R > 8.5$. The sample covering the whole sky, except the Milky Way zone, contains 490 UF galaxies with measured radial velocities. Our inspection of the neighboring galaxies around them revealed only 30 companions with radial velocity difference of $\mid\Delta V\mid<500$ km s$^{-1}$ inside the projected separation of $R_p < 250$ kpc. Wherein, the wider area around the UF galaxy within $R_p < 750$ kpc contains no other neighbors brighter than the UF galaxy itself in the same velocity span. The resulting sample galaxies mostly belong to the morphological types Sc, Scd, Sd. They have a moderate rotation velocity curve amplitude of about $120$ km s$^{-1}$ and a moderate K-band luminosity of about $10^{10}L_{\odot}$. The median difference of radial velocities of their companions is $87$ km s$^{-1}$, yielding the median orbital mass estimate of about $5\times10^{11}M_{\odot}$. Excluding six probable non-isolated pairs, we obtained a typical halo-mass-to-stellar-mass of UF galaxies of about $30$, what is almost the same one as in the principal spiral galaxies, like M 31 and M 81 in the nearest groups. We also note that ultra-flat galaxies look two times less "dusty" than other spirals of the same luminosity.

==> sao_cmd.tex <==
\def\saoname{Special Astrophysical Observatory of the Russian AS,
              Nizhnij Arkhyz 369167, Russia}
\def\saonamer{Специальная астрофизическая обсерватория, Нижний Архыз, 369167,
Россия}

%******* SPECIAL SIGNS AND CHARACTERS FOR MATH MODE *******
%
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\def\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\sun{\hbox{$\odot$}}

\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}

\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}

\def\degr{\hbox{$^\circ$}}

\def\arcmin{\hbox{$^\prime$}}

\def\arcsec{\hbox{$^{\prime\prime}$}}

\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}

\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}

\def\fd{\hbox{$.\!\!^{\rm d}$}}

\def\fh{\hbox{$.\!\!^{\rm h}$}}

\def\fm{\hbox{$.\!\!^{\rm m}$}}

\def\fs{\hbox{$.\!\!^{\rm s}$}}

\def\fdg{\hbox{$.\!\!^\circ$}}

\def\farcm{\hbox{$.\mkern-4mu^\prime$}}

\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}

\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}

\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}

\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}

\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}

\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}

\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}

\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}

\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}

\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}

\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}

\def\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\displaystyle/$}\hfil\crcr
{\hbox{$\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\textstyle/$}\hfil\crcr
{\hbox{$\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptstyle/$}\hfil\crcr
{\hbox{$\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}

\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}

%********** ABBREVIATIONS OF THE OFT-REFERENCED JOURNALS ***********

% *** Astrophysical Bulletin % англ. версия журнала САО с 2007 г.
\newcommand{\ab}{Astrophysical Bulletin}
% *** Астрофизический бюллетень % русск. версия журнала САО с 2007 г.
\newcommand{\abr}{Астрофизический бюллетень}
% *** Astronomy and Astrophysics
\newcommand{\aaa}{Astronom. and Astrophys.}
% *** Astronomy and Astrophys. Supplement Series
\newcommand{\aas}{Astronom. and Astrophys. Suppl. Ser.}
% *** Astronomy and Astrophysics Review
\newcommand{\aar}{Astronom. Astrophys. Rev.}
% *** Astronomical Journal
\newcommand{\aj}{Astronom. J.}
% *** Astrophysical Journal
%\newcommand{\apj}{Astrophys. J.}
% *** Astrophysical Journal Supplement Series
\newcommand{\apjs}{Astrophys. J. Suppl.}
% *** Astrophysics and Space Science
\newcommand{\apss}{Astrophys. and Space Sci.}
% *** Annual Review of Astronomy and Astrophys.
\newcommand{\araa}{Annu. Rev. Astronom. Astrophys.}
% *** Astronomicekij Zhurnal
\newcommand{\azh}{Astronom. Zh.}
% *** Bulletin of the American Astron. Society
\newcommand{\baas}{Bull. Amer. Astronom. Soc.}
% *** Bulletin of the Special Astrophysical Observatory % англ. версия до 2007 г.
\newcommand{\bsao}{Bull. Spec. Astrophys. Obs.}
% *** Бюллетень Спец. астрофизич. обсерватории % русск. версия до 2007 г.
\newcommand{\bsaor}{Бюлл. Спец. астрофиз. обсерв.}
% *** Inform. Bul. Var. Stars
\newcommand{\ibvs}{Inform. Bul. Var. Stars}
% *** Journal of Astronomy and Astrophysics
\newcommand{\jaa}{J. Astronom. Astrophys.}
% *** Monthly Notices of the Roy. Astron. Society
\newcommand{\mnras}{Monthly Notices Roy. Astronom. Soc.}
% *** Publ. Astronom. Soc. Japan
\newcommand{\pasj}{Publ. Astronom. Soc. Japan}
% *** Publ. of the Astron. Society of the Pacific
\newcommand{\pasp}{Publ. Astronom. Soc. Pacific}
% *** Pis'ma v Astronomicekij Zhurnal
\newcommand{\pazh}{Pis'ma Astronom. Zh.}
% *** Soviet Astronomy
\newcommand{\sovast}{Sov. Astronom.}
% *** Scientific American
\newcommand{\sca}{Scientific American}
% *** Sky and Telescope
\newcommand{\skytel}{Sky Telesc.}
% *** Space Science Reviews
\newcommand{\spsrev}{Space Sci.~Rev.}

